Beyond Latency: A System-Level Characterization of MPC and FHE for PPML

Privacy protection has become an increasing concern in modern machine learning applications. Privacy-preserving machine learning (PPML) has attracted growing research attention, with approaches such as secure multiparty computation (MPC) and fully homomorphic encryption (FHE) being actively explored. However, existing evaluations of these approaches have frequently been done on a narrow, fragmented setup and only focused on a specific performance metric, such as the online inference latency of a specific batch size. From the existing reports, it is hard to compare different approaches, especially when considering other metrics like energy/cost or broader system setups (various hyperparameters, offline overheads, future hardware/network configurations, etc.). We present a unified characterization of three popular approaches -- two variants of MPC based on arithmetic/binary sharing conversion and function secret sharing, and FHE -- on their performance and cost in performing privacy-preserving inference on multiple CNN and Transformer models. We study a range of LAN and WAN environments, model sizes, batch sizes, and input sequence lengths. We evaluate not only the performance but also the energy consumption and monetary cost of deploying under a realistic scenario, taking into account their offline and online computation/communication overheads. We provide empirical guidance for selecting, optimizing, and deploying these privacy-preserving compute paradigms, and outline how evolving hardware and network trends are likely to shift trade-offs between the two MPC schemes and FHE. This work provides system-level insights for researchers and practitioners who seek to understand or accelerate PPML workloads.

==> env.tex <==
% \usepackage{biblatex}
% \AtBeginBibliography{\small}
\usepackage{xcolor}
\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{authblk}
\usepackage{amsfonts}
\usepackage{stmaryrd}
\usepackage{marvosym}
\usepackage{lipsum}


\usepackage{makecell}
\usepackage[normalem]{ulem}
\let\labelindent\relax %for NDSS specifically
\usepackage{enumitem}
\newcommand{\ta}[1]{\textcolor{green}{\bf [takeaway: #1]}}
\newcommand{\ed}[1]{\textcolor{red}{\bf [ed: #1]}}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{pifont}
\newcommand{\change}[1]{\textcolor{red}{#1}}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{float}
\usepackage{svg}
\usepackage{biblatex}
\bibliography{BIBFILE.bib}

\usepackage{graphicx}
\usepackage{upgreek}


% \newcommand{\ph}[1]{\textcolor{green}{}}
\newcommand{\todo}[1]{\textcolor{red}{}}

==> intro.tex <==
\section{Introduction}

As machine learning (ML) becomes integral to daily activities, vast amounts of sensitive and private data are being processed by ML algorithms. In contexts such as medical applications, for instance, ML models may require access to private datasets distributed across different countries to make accurate predictions and decisions, often involving highly confidential health information \cite{kaissis2021end}. Similarly, cloud-based ML services, like those offered by major platforms such as Azure and Google AI, process user data using pre-trained models to deliver predictions and services \cite{Azure, GoogleAI}. However, this data, often containing sensitive personal details, is vulnerable to leakage and misuse.

While government regulations play a critical role in defining privacy policies, they alone cannot ensure comprehensive protection. The increasing risks of data breaches, cyberattacks, and unauthorized access make it clear that technical solutions are essential. Privacy-preserving machine learning (PPML) techniques offer robust protection, ensuring data confidentiality while still enabling the power of ML. By incorporating strong cryptographic protocols and privacy-focused mechanisms, PPML can safeguard sensitive information, allowing secure collaboration and data sharing across entities while minimizing the risk of data exposure.

One type of the major protocols used in PPML is the Secure Multiparty Computation (MPC or SMPC). Ever since the introduction of the first secure two-party computation protocol by Yao in 1982 \cite{yao1982protocols}, MPC has been widely studied and developed. In MPC, multiple parties collaborate to compute a function over their private inputs without revealing them to each other. The parties jointly compute the function output while keeping their inputs private. This is achieved by using cryptographic techniques such as secret sharing, homomorphic encryption, and garbled circuits. MPC has been applied to various ML tasks, including linear regression, logistic regression, neural networks, and deep learning \cite{mohassel2017secureml, mohassel2018aby3, wagh2020falcon, juvekar2018gazelle}.
